$C^3DRec$: Cloud-Client Cooperative Deep Learning for Temporal Recommendation in the Post-GDPR Era

Mobile devices enable users to retrieve information at any time and any place. Considering the occasional requirements and fragmentation usage pattern of mobile users, temporal recommendation techniques are proposed to improve the efficiency of information retrieval on mobile devices by means of accurately recommending items via learning temporal interests with short-term user interaction behaviors. However, the enforcement of privacy-preserving laws and regulations, such as GDPR, may overshadow the successful practice of temporal recommendation. The reason is that state-of-the-art recommendation systems require to gather and process the user data in centralized servers but the interaction behaviors data used for temporal recommendation are usually non-transactional data that are not allowed to gather without the explicit permission of users according to GDPR. As a result, if users do not permit services to gather their interaction behaviors data, the temporal recommendation fails to work. To realize the temporal recommendation in the post-GDPR era, this paper proposes $C^3DRec$, a cloud-client cooperative deep learning framework of mining interaction behaviors for recommendation while preserving user privacy. $C^3DRec$ constructs a global recommendation model on centralized servers using data collected before GDPR and fine-tunes the model directly on individual local devices using data collected after GDPR. We design two modes to accomplish the recommendation, i.e. pull mode where candidate items are pulled down onto the devices and fed into the local model to get recommended items, and push mode where the output of the local model is pushed onto the server and combined with candidate items to get recommended ones. Evaluation results show that $C^3DRec$ achieves comparable recommendation accuracy to the centralized approaches, with minimal privacy concern.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> Sections/backup.tex <==
A recommendation system learns users' interests and hobbies according to their profile or historical behaviors, and then predicts their ratings and hobbies for a given item \cite{shapira2015recommender}. Recently, temporal recommendation \cite{hidasi2015session, hidasi2016parallel, song2016multi, wu2017recurrent} has drawn much attention because user-item interactions usually contain timestamps and mining temporal information of interactions usually contributes to better performance of recommendation. As far as we are concerned, most of the existing approaches and industrial practices require to upload user behavior data from individual devices to the cloud server of recommendation service, where a recommendation model can be trained. Then, the prediction (or inference) process is performed either on the cloud or individual devices if the trained model is downloaded.

However, the above practices raise privacy issues. There are a considerable number of discussions about the possession, usage, and portability of user-generated data. Those public concerns about privacy leakage have gradually influenced policy and legislation formulation and eventually lead to General Data Protection Regulation (GDPR)\footnote{https://gdpr-info.eu/}, California Consumer Privacy Act (CCPA)\footnote{https://oag.ca.gov/privacy/ccpa/} and other privacy laws and regulations. GDPR states that a specific, freely-given, plainly-worded, and unambiguous consent should be given by the data subject, i.e. the user, and the data subject has the right of access, the right to data portability and the right to be forgotten. This means that, in the post-GDPR Era, if the user refuses to upload their behavior data to train a global recommendation model, the above approaches would be impractical.

Since the user behavior data produced \textit{after} GDPR cannot be uploaded without the user's consent, a straight forward solution is to take advantage of prior knowledge. DeepType \cite{xu2018deeptype} trains a global model on the cloud using massive public corpora, and then incrementally customizes the global model with data on individual devices, i.e. trains a personalized model for each user on his device. However, due to the heterogeneous of item metadata, i.e. item ID, category ID, there is few public dataset of cross-platform recommendation, to extract common prior knowledge for most recommendation systems, which means that we have to rely on existing behavior data collected \textit{before} GDPR to extract common knowledge. This raises the question of whether it complies with GDPR to process existing data collected \textit{before} GDPR. After carefully going through GDPR, we surprisingly find out that there is an exemption called Legitimate Interests\footnote{https://ico.org.uk/for-organisations/guide-to-data-protection/guide-to-the-general-data-protection-regulation-gdpr/lawful-basis-for-processing/legitimate-interests/} in GDPR which allows processing existing user data for legitimate interests without users' consent under careful consideration. The application scene of this mechanism includes fraud detection, crime prediction, network security protection, and marketing guidance, which means that the Legitimate Interests mechanism allows recommendation service to process user behavior data collected \textit{before} GDPR.

Inspired by related work and Legitimate Interests exemption of GDPR, we propose $C^3DRec$, a cloud-client cooperative deep learning framework for temporal recommendation in the post-GDPR era. First, we train a Recurrent Neural Network (RNN)\cite{mikolov2010recurrent} based global recommendation model with existing user behavior data collected \textit{before} GDPR for all users on the cloud, and push the global model to individual devices. Second, we train an RNN-based personalized recommendation model with real-time user behavior data collected \textit{after} GDPR for each user on his device, and extract a unique user embedding from his personalized model. Third, individual devices pull a recommendation item candidate set from the cloud (\textbf{pull mode}) or push user embeddings toward the cloud (\textbf{push mode}), and then we combine the latent information of user embeddings and item embeddings to complete the recommendation process. However, there are still two challenges we are supposed to tackle. To reduce network communication overhead between the cloud and devices, we perform the Least Absolute Shrinkage and Selection Operator (Lasso) regression\cite{tibshirani1996regression}, or $L_1$ regularization, to sparsify the item embeddings of item candidate set in pull mode or user embeddings in push mode. To reduce computational overhead on the devices, we perform an Automated Gradual Pruner (AGP)\cite{zhu2017prune} to compress the recommendation model.

To evaluate the performance of the proposed framework, we conduct experiments in terms of accuracy, communication overhead and computational overhead, based on a public user behavior dataset from Taobao\cite{zhu2018learning}, a large-scale e-commercial application in China, which contains nearly a million users and nearly 100 million interactions of users and items. The experimental results show that we achieve up to 10x reduction in communication overhead, reduce the computational overhead of on-device training towards the range of computational resources of middle-class mobile devices, with minimal loss in accuracy. We summary our contributions of $C^3DRec$ as follows.
\begin{itemize}
\item We propose an on-device deep learning framework for temporal recommendation, which alleviates the risks of user privacy leakage and violation of privacy-related laws, in benefit of recommendation service providers.
\item We reduce both communication and computational overhead of individual devices by AGP weight pruning and Lasso regression ($L_1$ regularization), to make sure that it is more feasible and less resource-consuming to perform on-device training of personalized models on real-world mobile devices, in benefit of application developers.
\item We evaluate the performance of $C^3DRec$ on a large-scale public dataset, and the experimental results show that we achieve up to 10x reduction in communication overhead and reduce the computational overhead towards the range of middle-class mobile devices, with minimal loss in accuracy.
\end{itemize}

The rest of the paper is organized as follows. In Section 2, we present the background of $C^3DRec$. In Section 3, we present the general framework of $C^3DRec$ and optimizations to reduce communication and computational overhead. Experiments and results are presented and discussed in Section 4. In Section 5, we discuss several limitations and future work of our framework. In Section 6, related work is presented and discussed. Finally, Section 7 concludes the paper.
